Environment Design for Reliable Shared Autonomy with Probabilistic Guarantees

Shared autonomy enables humans and robots to collaboratively perform tasks by combining human input with autonomous assistance. Most prior work focuses on improving intent inference under a fixed environment, overlooking how workspace design itself affects inference difficulty. We observe that the physical arrangement of objects directly influences the separability of candidate goals under noisy user inputs. We formulate workspace design as an optimization problem and derive a probabilistic correctness guarantee under a bounded noise model. Through simulation experiments across multiple tabletop scenarios, we show that optimized layouts improve goal inference reliability and reduce ambiguity compared to baseline arrangements. We further demonstrate a real-world shared autonomy system that integrates the proposed inference framework. This highlights the role of environment design as a complementary axis for improving shared autonomy systems.

==> experiments_intro.tex <==
\begin{figure*}[!ht]
\centering
\resizebox{0.92\textwidth}{!}{%
\begin{minipage}{\textwidth}
\centering
% First row: images
\begin{subfigure}{0.3\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/lunar_lander.png}
  % \caption{Lunar Lander}
\end{subfigure}
\hfill
\begin{subfigure}{0.3\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/tabletop.png}
  % \caption{Table Top}
\end{subfigure}
\hfill
\begin{subfigure}{0.3\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/navigation.png}
  % \caption{Navigation}
\end{subfigure}

\vspace{1em}

% Second row: table with horizontal lines
% \renewcommand{\arraystretch}{1.2}
\footnotesize
\begin{tabular}{@{}>{\centering\arraybackslash}p{0.1\textwidth} 
    >{\centering\arraybackslash}p{0.25\textwidth} 
    >{\centering\arraybackslash}p{0.3\textwidth} 
    >{\centering\arraybackslash}p{0.3\textwidth}@{}}
\toprule
 & \textbf{Lunar Lander} & \textbf{Table Top} & \textbf{Navigation} \\
\midrule
\textbf{Features $\Phi$} &
vertical speed, horizontal position &
objects that the end effector hovers over and the trajectory length &
path length, terrain traversed (paved, grass, asphalt and concrete)\\
\midrule
\textbf{Env params $\theta$} &
wind power, ranging from 1 to 20 &
object positions on the table &
terrain type of road network \\
\midrule
\textbf{Preferences} &
approach direction, landing speed &
objects to avoid hovering over &
terrains to avoid and path length \\
\bottomrule
\end{tabular}
\end{minipage}
} % end resizebox
\caption{Examples of preference queries with details and visualization across the three simulation domains. %feature vector $\Phi$, environment parameters $\theta$, and target preference or policy.
}
\label{fig:pref_queries}
\end{figure*}
